IMUTube: Automatic Extraction of Virtual on-body Accelerometry from Video for Human Activity Recognition

The lack of large-scale, labeled data sets impedes progress in developing robust and generalized predictive models for on-body sensor-based human activity recognition (HAR). Labeled data in human activity recognition is scarce and hard to come by, as sensor data collection is expensive, and the annotation is time-consuming and error-prone. To address this problem, we introduce IMUTube, an automated processing pipeline that integrates existing computer vision and signal processing techniques to convert videos of human activity into virtual streams of IMU data. These virtual IMU streams represent accelerometry at a wide variety of locations on the human body. We show how the virtually-generated IMU data improves the performance of a variety of models on known HAR datasets. Our initial results are very promising, but the greater promise of this work lies in a collective approach by the computer vision, signal processing, and activity recognition communities to extend this work in ways that we outline. This should lead to on-body, sensor-based HAR becoming yet another success story in large-dataset breakthroughs in recognition.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sec_1/intro_1.tex <==
On-body sensor-based human activity recognition is widely utilized for behavioral analysis, such as user authentication, healthcare, and tracking everyday activities~\cite{scholl2015wearables,Zhang12ubicomp,Chavarriaga13prl,Bachlin10titb,liaqat2019wearbreathing}.
Regardless of its utility, the human activity recognition field has yet to experience significant improvements over the past decades compared to other fields, such as speech recognition, natural language processing, and computer vision ~\cite{bao2004activity}. 
The ability in those domains to generate vast amounts of labeled data helps learn and evaluate models that can generalize to real-world datasets. 
However, collecting large-scale, labeled data sets has so far been limited in sensor-based human activity recognition. 
Labeled data in human activity recognition is scarce and hard to come by, as sensor data collection is expensive, and the annotation is time-consuming.
A model trained and evaluated on such a sparse dataset is difficult to generalize to a variety of real-world everyday activities.
Despite the numerous efforts in improving human activity dataset collection, the scale of typical datassets remains small thereby only covering limited sets of activities~\cite{Chavarriaga13prl,Zhang12ubicomp,thomaz2015practical,hovsepian2015cstress}. 
Even the largest sensor-based activity dataset spans tens of users with only a few weeks of recording~\cite{laput2019sensing}. 

In this work, we show that the hurdle for human activity data collection is possible to overcome.\thomas{Strong words. Maybe we should be a bit more humble here -- we show *one* way to overcome the problem.}
Fundamentally, we believe that the same information as with a real on-body inertial sensor can be captured from the human motion of individuals in the video. \thomas{It is not a matter of belief, is it?}
We show a way to collect a potentially large set of labeled human activity data by deriving virtual on-body sensor data from various human activity videos. \thomas{We may want to mention that these videos are retrieved in an opportunistic way, so basically from any data source we can get our hands on.}
We take visual information --just by watching people move-- and perform standard pose tracking and 3D scene understanding techniques. \thomas{No, *we* do not watch people move. We are only harvesting what is already out there but in a clever way -- which includes "labels".}
Then, activity classifiers are built with the full 3D human motion in the video, which are later tested on real IMU data.\thomas{It is not about the testing but about the eventual derivation of a sensor-based activity recognizer -- from data that are not real IMU data but rather opportunistically harvested data from large scale, curated video  repositories.}

As we adapt existing computer vision and graphics tools, the pipeline is fully automated and demands the minimum human labor.\thomas{We adopt rather than adapt, right? Also, this reference to human labor is not ideal.}
Since there are lots of readily available videos (namely youtube) we can dramatically increase the amount of sensor data available for a variety of activity recognition compared to the curated IMU datasets (e.g., PAMAP~\cite{reiss2012introducing}, Opportunity~\cite{Chavarriaga13prl}).
Recently some work also proposed virtual sensor datasets from 3D human motion generated by computer graphics rendering tools~\cite{kang2019towards}.
Differently from our work, such work is not entirely free from human labor costs, as they require human designers to create human motion as realistic as possible synthetically.
\thomas{What is the purpose of that last paragraph? It seems repetitive and also too low-level.}
\thomas{We jump straight to "pipeline" but never actually introduce and explain the big idea. The introduction should focus on the latter and not so much on technicalities ("pipeline").}

Through a series of experiments over three standard benchmarks datasets~\cite{sztyler2016body,reiss2012introducing,Chavarriaga13prl}, we demonstrate the viability of the proposed pipeline to produce useful virtual data for training a model to recognize activities from real sensor data. \thomas{Since the high-level idea was not properly introduced, this sentence is disconnected.}
Mainly, a model trained purely from virtual sensor data achieved acceptable performance (approximately 70\% of a model trained with real sensor dataset) on a real sensor dataset.
Moreover, only a few minutes of real sensor training data added to the virtual sensor data helped the model outperform the model trained on real sensor data in some scenarios. 
Collecting only a few minutes of real sensor data is trivial compared to the standard data collection protocol. 
\thomas{Add *here* why this matters.}

Importantly, this work broadly opens up many opportunities. 
The visual techniques used in the proposed pipelines are off-the-shelf and can be improved as the relevant computer vision, and graphic work further advances.
From abundant video sources online, the human activity community can acquire nearly labor-free large-scale datasets to train and evaluate deep learning models.
Also, we can freely conduct experiments on various on-body sensor configurations before collecting real sensor datasets.
Lastly, we expect the proposed data collection pipeline to accelerate the progress of human activity recognition research, as in other machine learning related fields.
\thomas{Move on from the focus on experiments. We have bigger fish to fry here: What are the implications for actual applications here?}

\thomas{Intro to end at end of page 2.}

==> sec_2/_related_work.tex <==
\section{Related work}

%\thomas{Missing: Intro that motivates why these methods are related work. What is the bigger picture here and what problems do all these methods try to solve -- just like we do?}
The proposed method details a pipeline towards opportunistically extracting virtual sensor data from a potentially very large body of publicly available videos. 
This is in contrast to current wearable sensor data collection protocols, which involve user studies and human participants, as well as other approaches that generate sensor data from motion capture (mocap) settings. 
In what follows, we first discuss approaches to data collection for sensor-based human activity recognition as well as mocap based techniques. 
These approaches represent the state-of-the-art in the field that are based on dedicated data recording protocols.
%\harish{(need a transition to go from one to the next. about how the previous protocols result in smaller annotated datasets)}. 
Subsequently, we detail prior work on training classifiers with limited labelled data, thereby focusing on data augmentation techniques and transfer learning. 

\subsection{Sensor Data Collection in HAR}
Sensor data collection for human activity recognition is performed by conducting user studies~\cite{Chavarriaga13prl,Zhang12ubicomp,reiss2012introducing}. 
Typically, the participants in a study are asked to perform activities in laboratory settings while wearing a sensing platform.
The advantage of data recording in a lab setting is that in addition to sensor data typically video data is recorded that is subsequently used for manual data annotation.
For this purpose, the sensor and video data streams need to be synchronized \cite{plotz2012automatic}, and human annotators need to be trained for consistency in annotation. 
The laboratory is designed to resemble a real-world environment, and user activities are either scripted or naturalistic. 
These include various gesture and locomotion level activities. 
However, designing a lab study to capture realistic natural behaviors is difficult. %\harish{need another word for this}. 
The protocol of such studies makes it challenging to collect large scale datasets. Furthermore, the annotation of activities is costly and error-prone and therefore prohibitive towards creating large datasets as they are required for deriving complex machine learning models. %\harish{uhh what am I doing here}
%\thomas{Unclear: Why is calling this out so important? What are the issues with that? Also unclear: what are the data? What are the labels? Where to labels come from? Paragraph seems a bit random here.}

Recently, Ecological Momentary Assessment (EMA) based approaches have been employed record and especially annotate real-world activity data \cite{laput2019sensing,thomaz2015practical,hovsepian2015cstress}. 
The sensing apparatus (containing sensors such as accelerometers or full-fledged IMUs) is worn on-body, and users self-report the activity labels when they are asked to do so through direct notification.
Although these methods may lose sample-precise annotation of the activities, they encourage the collection of larger scale datasets. 
While limited to gesture-based activities, Laput and Harrison \cite{laput2019sensing} have shown that larger numbers ($83$) of fine-grained hand activities can be reliably recorded and annotated.
%usable activity recognizers can be derived  using only a wrist sensor, if such data for model training is available. 
Both in-lab and EMA based collection protocols directly involve human participants to collect movement data using body-worn sensors. %\harish{(reads a bit off here but the idea is that real human participants are directly involved)}.

%Yet, either of in-lab or EMA-based data collection recruits participants to collect sensors from a real human. Not sure what Hyeok meant by this?
Other approaches have explored alternative data collection methods that do not directly involve human participants.
Kang \etal render a $3$D human model on computer graphics software 
%(e.g., Blender or Unity) 
and simulate human activities \cite{kang2019towards}. 
The sensor data is extracted from the simulated human motion, and subsequently used to train the recognition models. 
However, it is very difficult to realistically simulate and design complex human activities. 
Therefore, such methods typically only explore simple gestures and locomotion activities. %\thomas{True, but have you looked into robotics literature? They do a lot of simulation, which is decent. Applicable?}
Alternatively, ~\cite{xiao2020deep,takeda2018multi} extract sensory data from public, large-scale motion capture (mocap) datasets~\cite{mahmood2019amass,cmumocap,ofli2013berkeley}, which contain a variety of motions and poses for human activity recognition. 
Although these datasets cover hundreds of subjects and thousands of poses and motions, they rarely include everyday activities. 
The majority of such mocap datasets include dancing, quick locomotion transitions, and martial arts, which are less relevant to recognizing daily human activities.

\hyeok{Most related to our work, Rey~\etal~\cite{rey2019let} also have proposed to collect virtual sensor data from online videos, and showed the virtual sensor useful for recognizing fitness activity.
Their approach collects 2D pose motion for a single person in the video with fixed camera viewpoint. 
From the synced video and accelerometer recording, the changes in joint locations in 2D scene is regressed to the norm of three-axis accelerometer.
With the similar motivation, we extend their work to the full 3D motion estimation from the video with the multiple people and camera motion tracking.
Our approach do not require synced video and wearable recording for domain shift from virtual sensor to real sensor.

Therefore, our method can extract full IMU information (three-axis accelerometer, gyroscope, and simulated magnetometer) for any wild video for human activity recognition.}

% Hence, evaluated activity classes are limited to locomotion and simple gesture motions for supervised model training with virtual sensor streams. Not sure what Hyeok means here.
%In the case of complex activities, these works mainly utilize the extracted sensor data for the unsupervised pretraining of the deep models for representation learning, which are then fine-tuned with real sensor data for target activities~\cite{xiao2020deep}. In 
%They can further scale the extracted dataset by modifying 3D human character with different height and body part ratio [seems to come out of nowhere].
%\thomas{I do not understand the relevance of this last, short paragraph.}

In this work, we instead leverage the availability of large scale video datasets that cover real-world activities to extract sensory data. 
These videos are recorded in-the-wild and contain a wide range of activities, including everyday activities, which makes them very attractive for deriving realistic and robust human activity recognition systems.
%This allows us to avoid artifically simulating $3$D human characters or limiting activities to those available in the mocap datasets.
%In this work, we propose a data collection pipeline that leverages the publicly available large scale video data, while avoiding artificially simulating $3$D human characters or limiting activities to those available in the mocap datasets. %\thomas{I am pretty sure this sentence is wrong. "Vast availability and scale of virtual sensor data"? That's our actual contribution!}
%To acquire real human behavior, we compute virtual sensor data for human motion from freely available online video platforms, which contain vidoes recorded in the wild. By leveraging approaches from computer vision and graphics domains, we estimate the full $3$D motion of individuals present in the video segments. %Our approach can also modify estimated $3$D human motion to various height and body part ratio and extract sensor data from any arbitrary body location, similarly with the abovementioned approaches.
%\thomas{Why having this summary *here"? Distracting.}

%\harish{add something about how datasets end up being smaller in size so that we can transition to why augmentation etc is actually required.}


\subsection{Tackling the Sparse Data Problem}
%\thomas{We are making a conclusion here on something we have not spelled out: labelled dataset for HAR are small. Where in the previous section have we actually made that point?}
%\edited{As the labelled datasets for human activity recognition from body worn sensor data tend to be smaller relative to other domains such as vision or natural language, prior works use data augmentation techniques as they prevent overfitting, and improve the generalizability of deep learning models \cite{ Goodfellow-et-al-2016}} . 
%\thomas{No, don't make this about DL.}
Many publicly available datasets for human activity recognition contain imbalanced classes. For example, approximately $75\%$ of the Opportunity dataset (which has $18$ classes in total) \cite{Chavarriaga13prl} consists of the null class \cite{guan2017ensembles}, making it challenging to design classifiers. The activities being studied also impact the class imbalance to some extent. In the PAMAP2 dataset, the skipping rope class constitutes approximately $2.5\%$ of data, relative to other activities which constitute around $9\%$ on average \cite{guan2017ensembles}. 
This follows reason as %, unless your name is Rocky Balboa, 
it is harder for subjects to perform rope skipping for longer durations of time, in contrast to walking or lying down. 
This resulting class imbalance poses a challenge for the design and training of classifiers, which may find it easier to simply predict the majority class. 
Furthermore, the relatively small size of labelled datasets results in models quickly overfitting and does not allow application of complex model architectures. 
It is also difficult to apply potentially alleviating techniques such as transfer learning, which rely on large datasets for knowledge transfer. 
%\harish{is there something else we can talk about for small dataset issues?}

As a way to overcome the problem of small,  class-imbalanced datasets, data augmentation techniques have been applied previously to prevent overfitting, improve generalizability and increase variability in the datasets. 
They involve techniques that systematically transform the data during the training process in order to make classifiers more robust to noise and other variations \cite{mathur2018using}. 
%\thomas{What does "enrich" mean?}\harish{well here it is meant to convey that the training data is `enhanced' to contain more variations that could possibly help with test metrics.}
They artificially inflate the training data by utilizing methods, which perform data warping, or oversampling \cite{shorten2019survey}. 
Data warping includes geometric transformations such as rotations, and cropping, as well as adversarial training. 
Meanwhile, oversampling involves feature space augmentations and generative adversarial networks (GANs) \cite{shorten2019survey}. 
For time series classification, the data warping techniques include window slicing, window warping, rotations, permutations and dynamic time warping \cite{le2016data, fawaz2018data}. 
Several of these transformations can be combined to further improve the performance over a single method. 
Um~\etal~demonstrate that combining three basic methods (permutation, rotation and time warping) yields better performance than using a single method \cite{ um2017data}. 
In \cite{rashid2019times}, construction equipment activity recognition is also improved by combining simple transformations. 

Oversampling based methods include synthetic minority oversampling technique (SMOTE) \cite{ fernandez2018smote} which addresses the class imbalance problem by oversampling, and GANs, which are, for example, used for augmenting biosignals  \cite{ haradal2018biosignal}. 
In \cite{ramponi2018t}, a data augmentation technique for time series data with irregular sampling is proposed utilizing conditional GANs. 
It is shown to outperform data warping techniques such as window slicing and time warping. 
%\thomas{First time we mention class imbalance, which makes me think that we have never explained why the small datasets actually are a problem. Harish can speak volumes to that and I suggest we should have a clarification section here in section 2 that elaborates on what the issues are with small datasets. }
Augmentation for wearable sensor data has been explored for monitoring Parkinson’s disease in \cite{um2017data}. 
In this paper, seven transformations, including jittering, scaling, rotation and warping are detailed and their effect relative to no augmentation is studied. 
Further, the authors observed that combining multiple transformations results in higher performance. 
In \cite{steven2018feature}, augmentation is performed on IMU spectrogram features to improve the activity recognition performance. 

Another approach to deal with small labelled datasets includes transfer learning. 
Here, a base classifier (typically a neural network) is first trained on a base dataset and task. 
Subsequently, the learned features are re-purposed, or \emph{transferred}, to a second target network to be trained on the target dataset and task. 
In particular, if the target dataset is significantly smaller compared to the base dataset, transfer learning enables  training a large target network without overfitting \cite{yosinski2014transferable}, and typically results in improved performance. 
%\thomas{Explain what transfer learning is.}
In \cite{saeed2019multi}, the authors propose a self-supervision pretext task and demonstrate its effectiveness for unsupervised transfer learning on other datasets with little labelled data. 
A more extreme example of having very small labelled datasets includes one-shot and few-shot learning, which contain very few labelled samples per class \cite{feng2019few}.

While the data augmentation techniques do improve the classification performance, they, ultimately, produce perturbed training samples. 
Therefore, they are unable to provide for the variety in human movements that is obtained by collecting data from a large number of subjects. 
On the other hand, the GAN based techniques perform augmentation by sampling from the dataset distributon. 
However, they require substantial amounts of data to train, and suffer from training instability and non-convergence. 
Furthermore, there is limited prior work studying data augmentation by GANs for wearable sensor data and their actual suitability for sensor-based human activity recognition remains to be shown.
This makes it challenging to readily apply these generative networks to create more data. 

We tackle the problem of having small labelled datasets with a different approach -- by generating large quantities of virtual IMU data from videos. 
As we can leverage a large body of videos, containing many individuals, we generate datasets containing more diverse movements and potentially much larger datasets of realistic data, which is in stark contrast to existing methods that try to combat the sparse data problem.
%relative to both augmentation and GANs. 
%\thomas{I think we should extend this last paragraph as it reflects nicely and sets the scene for the gist of the paper. Maybe even make it a subsection here.}


==> sec_3/figures/pose_estimation.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}[t]{@{\hspace{-0.25cm}} c}
    \includegraphics[align=c,width=0.7\linewidth]{./sec_3/figures/pose_estimation.png}
    \vspace{-0.0in}
\end{tabular}
\end{center}
\vspace{-0.15in}
\caption{The 3D joint orientation estimation from the video.
The multi-person 2D poses are estimated with \emph{OpenPose} model which 2D poses are lifted to 3D poses with \emph{VideoPose3D} model.}
\label{fig:pose} 
\vspace*{-1em}
\end{figure}

==> sec_3/method_1.tex <==
\input{./sec_3/figures/overall.tex}
%\thomas{Better title needed. We are describing a radically different way to derive HAR systems, it is not about a data collection system.}
\thomas{We need to actually introduce the overall idea of this paper and not jump straight into technical details. Also, and importantly: We do not link the video processing pipeline to HAR -- which, however, is the whole point of this paper. The figure is way too low-level and only focuses on the CV related steps. What we want to introduce in this paper, however, is not merely a computer vision pipeline just for the sake of it but rather a means to end for improved sensor-based activity recognition. We need to show this in the figure and describe this overarching idea here in the intro to this section. Then and only then we can jump deep into the technical details.} \nic{yes, i agree here. i imagine this to be sec 2. and it provides a more conceptual view of what and fleshes out in a bit more detail what is setup in the introduction. i imagine something that has a conceptual (simplified) series of components, use cases/opportunities (some of which are realized nearly realized in this paper, others which are pending -- like the creation of big data set). and perhaps hints at challenges. it might relatively brief. Perhaps a nice way to break this with the detail you have here is to have a conceptual section followed by a algorithms section in which you detail what it is in this paper that has been done and how it currently is designed. that way you have a separate place to convey the 'ideas' and then you have a place to convey what we have working at this minute.}\nic{this can also be a place to be very deliberate in introducing the term 'virtual imu' and 'real imu' as we rely on them so much in the paper. we want the reader to know clearly what is meant}

In this work, we propose to utilize the human activity videos as sources to learn inertial motion when an activity is undertaken.
Inertial sensors include not only the local joint orientation and position change, but also the global bodily movement over time in 3D world.
Hence, both motion information shall be estimated from the sequence of 2D snapshots (frames) of the activity.
As shown in \figref{fig:overall}, let's consider a video in which a person is riding on a bicycle, and which camera is following the person centering in the frame.
From this video, naively estimating 3D pose from each frame would result in a static posture with zero acceleration, if the global camera ego-motion is not considered.
A global 3D scene structure across frames is also necessary to estimate the 3D human motion accurately integrating the person's 3D pose, localization per frame, and global camera ego-motion across frames.
Although the third dimensional information is inherently uncertain from 2D video, the computer vision community has recently had the significant progress in disambiguating the 3D information from the various 2D scenes in the wild.
Once full 3D motion is estimated, then the virtual on-body sensor stream is extracted from each 3D person.
The virtual sensor is expected to contain the 3D inertial motion which also a real sensor would have been captured if attached on the person in the video.
Hence, we propose training a recognition model on the collection of virtual sensor, instead.

Next, we introduce the technical overview and details of the data collection pipeline shown in the \figref{fig:overall}.
Before moving on, we note that the online video can typically be a concatenation of different video clips from different people, even though the entire video sequence includes the activity of interest. 
Thus, the scene boundary detection~\cite{HassanienESHM17} is firstly applied to extract multiple clips of separate activity sequences.
Then, virtual sensor sequences are extracted from each video clip.
From a video clip, the abovementioned two different 3D scene information is estimated, which are 3D pose (local joint motion) and the global body motion of the people.

% In the following section, we discuss the technical procedures of 1) 3D pose and localization, and 2) camera ego-motion estimation.
%\thomas{See my comment above: This is not the appropriate level for an overview that shall explain the big picture.}

\subsection{3D joint motion estimation}
\input{sec_3/figures/pose_calibration}

% \thomas{Unclear: Why do we do all that. 
% Start these subsections with a description of the specific goal. 
% Why would we be interested in poses, for example. It may sound trivial but the point we are trying to make here is not to convince the reader that we know how to do computer vision but rather that 
% we have a clever idea to overcome those issues related to training a HAR system -- so, always keep the connection to that big idea.}

Since the on-body sensors captures the local 3D joint motion, we also extract the joint motion from 2D video through popularly used 2 step approach as shown in \figref{fig:pose}.
First of all, we estimate 2D pose skeletons for multiple people in the scene with \emph{Openpose} model~\cite{cao2017realtime}.
Each 2D pose will be lifted to 3D pose afterward. 
In this work, we assume that all people in the scene are on-going the same activity with different motions.
Although fast and accurate, the \emph{Openpose} model estimates 2D poses of people frame by frame, so that person ID for the same person does not match across the frames.
Hence, we apply the \emph{SORT} tracking algorithm~\cite{Bewley2016_sort} to track each person across the frame.
\emph{SORT} utilized bipartite graph matching with the edge weights as intersection-over-union (IOU) distance between boundary boxes of people from consecutive frames.
The boundary boxes are derived as tight box including 2D keypoints for each person.

To increase the reliability of 2D pose detection and tracking, we remove 2D poses with over half of the joints are missing, and also ignore the tracked sequence shorter than a second.
For each tracked person sequence, we also interpolate and smooth missing or noisy keypoints in each frame using a Kalman filter, as poses between a fraction of a second cannot be dramatically different.
Capturing inherent smooth transition of 2D poses across the frame has encourage more natural 3D motion in the finally estimated (lifted) 3d pose.
%\thomas{Again, motivate and explain why we are doing all this.}
Lastly, each 2D pose sequence is lifted to 3D pose with \emph{VideoPose3D} model~\cite{pavllo20193d} which local 3D joint rotation for virtual sensor is extracted.
%\thomas{Why?}

\subsection{Global body location tracking in 3D}

As mentioned earlier, inertial sensors captures the acceleration from global body movement in 3D space, additionally to the local joint motion.
Thus, we also have to extract global 3D scene information from 2D video to track the person's movement in the whole scene.
Typical 3D pose estimation models do not localize the global 3D position and orientation of the pose in the scene. 

The 3D person tracking in 2D video requires two information, which are 3D localization in each 2D frame, and the camera viewpoint changes (ego-motion) between subsequent 3D scenes. 
Briefly, the tracking algorithm maps the 3D location of a person of a frame to the corresponding position within the whole 3D scene in video, according to the camera viewpoint of the frame. 
The sequence of the location and orientation of 3D pose is the global body movement in whole 3D space.
For the virtual sensor, the global acceleration from tracked sequence will be integrated with local joint acceleration.

\subsubsection{Calibrating 3D pose in the frame}
\hfill\\
The first step to acquire 3D movement in whole 3D scene sequence is to estimate 3D rotation and translation of a 3D pose within a frame.
For each frame, we calibrate each 3D pose from previous 3D joint estimation according to the perspective projection between corresponding 3D and 2D keypoints, as shown in \figref{fig:pose}.
The perspective projection can be estimated with the Perspective-n-point (Pnp) algorithm~\cite{Hesch_2011}.
Additionally to 3D and 2D correspondences, the Pnp algorithm requires the camera intrinsic parameters for the projection, which include focal length, image center, and the lens distortion parameters~\cite{Shah_1996,Caprile_1990}.
Since arbitrary online video typically does not provide EXIF metadata, the camera intrinsic parameters are estimated from the video with \emph{DeepCalib} model~\cite{Bogdan_2018}.
The \emph{DeepCalib} model is a frame-based model that considers a single image at a time so that the estimated intrinsic parameter for each frame slightly differs across the frame according to its scene structure.
Hence, we assume that a given video clip sequence is recorded with a single camera, and aggregate the intrinsic parameter predictions by taking the average from all the frames.
%\thomas{Some of these technical details and necessities may be better explained with an illustration.}

\begin{equation}
    \begin{gathered}
        c^{int} = \frac{1}{T}\sum_{t=1}^T c^{int}_t
    \end{gathered}
\end{equation}

\noindent where, $c^{int}=[f,p,d]$ is averaged camera intrinsic parameters from each frame at time $t$, $x_t$, predictions, $c^{int}_t=DeepCalib(x_t)$. $f=[f_x,f_y]$ is focal length and $p=[p_x,p_y]$ is optical center for $x$ and $y$ axis, and $d$ is lense distortion.
Once the camera intrinsic parameter is calculated, Pnp algorithm regress global pose rotation and translation by minimizing the following objective function, $J$,

\begin{equation}
    \begin{gathered}
        \{ R^{calib}, T^{calib} \} = \arg\min_{R, T} \sum_{i=1}^N \| p^i_2 - \frac{1}{s} c^{int} (R p^i_3 + T) \| \\
        \text{subject to } R^T R = I_3, det(R) = 1
    \end{gathered}
\end{equation}

\noindent where $p_2 \in \mathbb{R}^2$ and $p_3 \in \mathbb{R}^3$ are corresponing 2D and 3D keypoints, accordingly.
$R^{calib} \in \mathbb{R}^{3 \times 3}$ is extrinsic rotation matrix, $T^{calib} \in \mathbb{R}^3$ is extrinsic translation vector, and $s \in \mathbb{R}$ is scaling factor~\cite{Qilong_Zhang,Zhuang_1995}.
For the temporally smooth rotation and translation of 3D pose across the frames, we initialize the extrinsic parameter, $R$, and $T$, with the result from the previous frame.
The 3D pose for each person, $p_3 \in \mathbb{R}^{3 \times N}$, at each frame is calibrated (or localized) with the estimated corresponding extrinsic parameter.

\begin{equation}
    p^{calib}_3 = R^{calib} p_3 + T^{calib}
\end{equation}

\noindent From the calibrated 3D poses, $p^{calib}_3 \in \mathbb{R}^{3 \times N}$, we remove people considered as the background.
Depending on the scene, all the people in the scene may not part-take in the activity.
For example, for rope jumping competition scene, a set of a person may rope jumping while others are sitting and watching.
To effectively collect 3D pose and motion that belongs to the target activity, we should remove those background people.
We first calculate the pose variation across the frames as the summation of the variance of each joint location across time.
Afterward, we keep the people with the pose variation larger than the median of all people and remove the rest.

\subsubsection{Camera egomotion estimation}
\hfill\\

\input{sec_3/figures/pose_egomotion}

In arbitrary online video, the camera can move around the scene freely.
However, the pipeline should not confuse the camera motion with human motion.
For example, a person with static pose can appear in different location in the subsequent frames according to the camera movement.
Also, a moving person can always appear in the center of the frame if the camera follows the person.
In these two cases, the virtual sensor should capture static motion or the global body acceleration, respectively, regardless of camera motion.
Hence, before extracting virtual sensor, the previously calibrated per-frame 3D pose should be compensated with the camera ego-motion (the viewpoint change) across the frames.

Camera ego-motion estimation from one camera viewpoint to another needs 3D point clouds of both scenes~\cite{Rusinkiewicz,Besl_1992,Pomerleau_2015}.
Deriving a 3D point cloud of a scene needs two information, which is the depth map and camera intrinsic parameters.
For camera intrinsic parameter, we reuse the previously estimated parameters.
The depth map is the distances of pixels in the 2D scene from the given camera center, which we estimate with the \emph{DepthWild} model~\cite{Gordon_2019} for each frame.

Once we have a depth map and camera intrinsic parameter, we can geometrically inverse map each pixel in the image to the 3D point cloud of the original 3D scene.
With basic trigonometry, the pointcloud can be derived from the depth map using the previously estimated camera intrinsic parameter, $c^{int}=[f_x, f_y, p_x, p_y, d]$. For depth value $Z$ at image position $(x,y)$, point cloud value, $[X, Y, Z]$, is

\begin{equation}
    [X, Y, Z] = \Big[\frac{(x-p_x) \cdot Z}{f_x}, \frac{(y-p_y) \cdot Z}{f_y}, Z \Big]
\end{equation}

\noindent Now that point clouds across frames are calculated, we derive the camera ego-motion (rotation and translation) parameter between two consecutive frame point clouds.
A group of the algorithm named Iterative Closest Points (ICP) is widely utilized for registering a group of point clouds~\cite{Rusinkiewicz,Besl_1992,Pomerleau_2015}.
Fixing a point cloud as a reference, ICP iteratively finds closest point pairs between two point clouds and estimate rotation and translation for the other point cloud that minimizes the positional error between matched points~\cite{Besl_1992}.
Since we have colored point cloud from the given image, we adopted Park~\etal~\cite{park2017colored}, which considers color matching between the matched points additionally to the surface normals to enhance color consistency after the registration. 
Here, we utilize background point clouds instead of the entire point cloud from the scene.
The observational changes for the stationary background objects in the scene are more relevant to the camera movement.
We consider humans in the scene are foreground objects, and remove points that belong to human bounding boxes from 2D pose detection.
We observed including foreground objects, such as humans, confuses ICP algorithms between the motions from the moving objects (humans) and camera.
With the background point clouds, we apply colored ICP algorithm~\cite{park2017colored} between pointcloud at time $t-1$ and $t$, $q_{t-1}$ and $q_t$ respectively. 
We iteratively solve,

\begin{equation}
    \{ R^{ego}_t, T^{ego}_t \} = \arg\min_{R, T} \sum_{(q_{t-1}, q_t) \in \mathcal{K}} (1-\delta) \|\mathcal{C}_{q_{t-1}}(f(Rq_t + T)) - \mathcal{C}(q_{t-1})\| + \delta \|(Rq_t + T - q_{t-1}) \cdot n_{q_{t-1}} \|
\end{equation}

\noindent $\mathcal{C}(q)$ is the color of point $q$, $n_q$ is the normal of point $q$. 
$\mathcal{K}$ is the correspondence set between $q_{t-1}$ and $q_t$, and $R^{ego}_t \in \mathbb{R}^{3 \times 3}$ and $T^{ego}_T \in \mathbb{R}^3$ are fitted rotation and translation vector in the current iteration. 
$\delta \in [0, 1]$ is the weight parameter for the balance between positional and color matches.

The estimated sequence of translation and rotation of point cloud is the resulting ego-motion of camera viewpoint from the video.
Finally, we integrate the estimated 3D pose, camera extrinsic, and ego-motion across the video to fully track 3D human motion.
Previously calibrated 3D pose sequence, $p^{calib}_3$, are rotated and translated according to its ego-motion at frame $t$.

\begin{equation}
    p^{track}_{3_t} = R^{ego}_t p^{calib}_{3_t} + T^{ego}_t
\end{equation}

\noindent $p^{track}_3 \in \mathbb{R}^{T \times N \times 3}$ is the resulting 3D human pose and motion tracked in the scene for the video, where $T$ is the number of frames, and $N$ is the number of joint keypoints.
The overall process is illustrated in \figref{fig:ego_motion}.

\subsection{Virtual sensor simulation and extraction}
%\nic{it feels like there is too much attention to 3.1 and 3.2 and not enough to stages that happen afterwards like in 3.3 and 3.4}

Now that we have full 3D motions for each person in the video, we extract sensor streams from the interested on-body location.
The estimated 3D motion only gives the location of each joint keypoints.
However, to track the local sensor coordinate rotation while moving, we also need to track the orientation change of the local joint, on which the sensor is attached.
The local joint orientation changes can be calculated with the forward kinematics from the hip (the body center) to each joint, which function is provided by 3D animation software (e.g., blender).
Using the orientation derived from forward kinematics, the acceleration of joint movements in the world coordinate system will be transformed into a local sensor coordinate system.
The angular velocity of the sensor (gyroscope) is calculated by tracking the orientation changes of the sensor.

Lastly, we utilize the \emph{Imusim}~\cite{YoungLA11} model to extract realistic sensor behavior for each interested on-body location.
\emph{Imusim} estimates sensor output considering mechanical and electronic components in the device, as well as the simulated magnetic field change in the environment. 
Compared with real IMUs, \emph{Imusim} has empirically outperformed the naive approach deriving the acceleration or velocity with position derivatives.
Hence, it has been applied for a number of gait analyses with virtual characters in biomechanical community~\cite{Phm2018SplineFS,Karlsson14inertial,bodynets}.
We note that previous virtual sensor data collection in the human activity recognition community utilized a naive approach based on position derivatives.

\subsection{Sensor distribution adaptation}

Although the extracted sensor stream may capture the core temporal patterns of the target activity in the estimated 3D motion, the intrinsic characteristic of the virtual sensor can be far from that of the actual physical sensor used for the activity recognition.
As the last step before using a virtual sensor dataset for the model training, we transfer the distribution of the virtual sensor to that of the target sensor.
For computational efficiency, the rank transformation approach~\cite{conover1981rank} is utilized.

\begin{equation}
    x_r = G^{-1}(F(X \leq x_{v}))
\end{equation}

\noindent where, $G(X\leq x_r) = \int_{-\inf}^{x_r} g(x) dx$ and $F(X\leq x_v) = \int_{-\infty}^{x_v} f(x) dx$ are cumulative density functions for real, $x_r$, and virtual, $x_v$, sensor samples, respectively.
In the experiment, we will show that only a few seconds to minutes of a real sensor stream is enough to transfer the virtual sensor effectively for the activity recognition, which amount is trivial to collect.


==> sec_4/experiment.tex <==
We evaluate the validity of the proposing data extraction pipeline through several activity recognition tasks on benchmark real sensor datasets.
The model trained with the virtual sensor will perform similarly as the model trained with real sensor data if the virtual sensor dataset from videos captures real-world human behavior.
Hence, we compare the model trained with our virtual dataset with the baseline model trained with a real sensor dataset, testing on the test set from the corresponding benchmark real sensor datasets.

\subsection{Datasets}

Among publicly available sensor datasets, Realworld~\cite{sztyler2016body}, PAMAP2~\cite{reiss2012introducing}, and Opportunity~\cite{Chavarriaga13prl} datasets are used to evaluate the model across simple (locomotion) to complex (home and sports) activities.
For each dataset, the train, validation, and test split are chosen according to the previous benchmark work unless mentioned otherwise.
For the Opportunity dataset, we choose four locomotion level classes for the experiment. The middle and high-level activity classes are too specific or broad for searching the corresponding video activities, respectively.
For each Opportunity, PAMAP2, and Realworld dataset, the samples from subject 4, 6, 15 were held out for test sets, respectively.

For the virtual sensor dataset, we find the video sources for the activity classes in the sensor benchmark dataset.
All three benchmark datasets have locomotion activities. 
Especially, the Realworld dataset includes the video recordings taken while 15 subjects performing the eight locomotions, which are \emph{climbing down, climbing up, jumping, lying, running, sitting, standing}, and \emph{walking}.
For the locomotion activities, the virtual sensors extracted from Realworld videos are utilized for all the experiments.
On the other hand, the PAMAP2 dataset includes other complex activities, which are \emph{cycling, vacuum cleaning, ironing}, and \emph{rope jumping}, according to the benchmark experiment~\cite{Hammerla16ijcai}.
For those four activities, we utilize the corresponding video segments from multiple benchmark video activity datasets, which include ActivityNet~\cite{caba2015activitynet}, Kinetics700~\cite{carreira2019short}, HMDB51~\cite{kuehne2011hmdb}, MPIIHPD~\cite{andriluka14cvpr}, UCF101~\cite{soomro2012ucf101}, Charades~\cite{sigurdsson2016hollywood}, AVA~\cite{gu2018ava}, MSRdailyactivity3D~\cite{5543273}, and NTU RGB-D~\cite{Liu_2019_NTURGBD120}.

[figure for bar chart comparison between real and virtual IMU]

\subsection{Evaluation Protocol}

We largely explored two different approaches for utilizing a virtual sensor dataset.
In first experiment, the real sensor training dataset is either replaced or mixed with virtual sensor dataset for supervised model training.
For supervised learning, both shallow and deep learning models are evalutaed, which are Random forest (RF) with ECDF feature~\cite{hammerla2013preserving} and ConvLSTM model~\cite{Ordonez16sensors}.
Secondly, we analyze the utility of virtual sensor representation for arbitrary real sensor dataset with the domain transfer learning.
The model initially learns the sensor representation trained for virtual sensor data with or without its labels. 
ConvLSTM model is used for the supervised pretraining, and the autoencoder (AE) with MLP is used for the unsupervised transfer learning.
Then, the model is fine-tuned with a small subset of the target real sensor dataset with the labels for classification.

For deep learning model training, we followed the standard hyperparameter tuning protocol using a held-out validation set with a grid search.
The learning rate was searched from $10^{-6}$ to $10^{-3}$, and weight decay was searched from $10^{-4}$ to $10^{-3}$. 
Lastly, we used the mean F1 score, and Wilson score interval~\cite{wilson1927probable} for the statistical significance of performance difference.

% the limitation of system
% limitations
% not all people do the same action
% label is hard to get (classifier)

\subsection{Results}

\input{sec_4/tables/all}

First of all, RF and Convlstm are supervised trained with virtual sensor data either alone (Virtual-to-Real: V2R) or mixed with real sensor data (Mixed-to-Real: M2R). 
Afterward, transfer learning results are shown.
The Convlstm is supervised pretrained (Supervised-Transfer-to-Real: ST2R), and AE is unsupervised  (Unsupervised-Transfer-to-Real: UT2R) pre-trained with the virtual sensor. 
Both Convlstm and AE are fine-tuned with small samples of real sensor datasets.
For all experiments, the proposed model is compared with the baseline model trained with real sensor data (Real-to-Real: R2R).

\subsubsection{Supervised model training with virtual sensor}
\hfill\\

Here, we evaluate if the virtual sensor can replace the real sensor for supervised model training, and if not, how much real sensor data is required.
\tblref{tbl:summary} shows the summary of the model performances for a different training scheme with a virtual sensor dataset compared to the model trained with a fully available real sensor dataset (R2R).

Across dataset and models, the V2R model achieves approximately 70\% of the corresponding R2R model performance.
When labeled real sensor sample is available (M2R), the model performance increases as expected and matches up to 90\% of the corresponding R2R model performance.
For M2R, we used 10 minutes of real sensor data for each activity for model training, additionally to the virtual sensor data.
When trained along with a virtual sensor dataset, the required real sensor data collection is trivially small compared to entirely relying on real sensor data, which requires hours data collection across multiple people.

\input{sec_4/figures/rf_dl}

As utilizing real sensor data added to the virtual sensor is helping (M2R), we investigate the performance difference according to the different amounts of real and virtual sensor data.
In \figref{fig:supervised}, we compared R2R, V2R, and M2R models with different duration of corresponding sensor type training samples from 1 second to 10 minutes.
Either RF or Convlstm, M2R outperformed the V2R model for any training sample size.
For a simple classification task (Realworld, 8 locomotions), a model trained with more or less a minute of virtual and real sensor training set (M2R) could surpass the model trained with a full real sensor dataset.
Even when only using a virtual sensor training dataset (V2R), 10 minutes of data was enough to match the performance of the R2R full dataset model.

\subsubsection{Transfering representation from virtual to real sensor}
\hfill\\

\input{sec_4/figures/tl}

In \tblref{tbl:summary}, the ST2R model outperforms both of the R2R and M2R models.
ST2R model can benefit from the rich discriminative sensor representation learned from all available labeled virtual sensor data.
Such effective sensor representation can significantly reduce the amount of real sensor data to adapt to the target classification task.

\figref{fig:dl_tl} shows the performance of the ST2R model fine-tuning with different amounts of real sensor datasets.
For both Realworld and PAMAP2-11 datasets, ST2R requires less than 10 minutes of real sensor data was enough to surpass the R2R model trained with a full real sensor full training dataset.
Especially ST2R was more effective when the target task was simple (Realworld, 8 locomotions).

\textcolor{red}{[analysis UT2R after filling the table (Harish is running the experiment.)]}



%--- where Catherine left off May 10th
%--- Hyeok reflected them in the updated version.
% In this section, we describe the design and results of our investigations carried out to validate the proposed pipeline.

% \subsection{Design}
% While our ultimate vision is to to apply the pipeline to any videos, in this work we focus on two specific video collection protocols. They are designed to demonstrate the potential of our pipeline under circumstances which are of the most interest to the HAR community.

% \textbf{Time-synchronized Video-IMU data} {}
% We wish to compare two sources of information describing the exact same activities under the same settings. Realworld dataset provides such a platform: it contain videos of 15 subjects performing each activity while wearing motion sensors. Although in this dataset the video and IMU data streams were not perfectly synchronized, we can compare the visual-generated virtual data and real IMU data while holding activities constant. This gives us video data of 8 locomotion activities. In addition, the HAR community is familiar with the realworld dataset and its activity labels (all locmotions) are commonplace in other popular HAR datasets. 

% % data distribution plots. 

% \textbf{Manually-curated video data} {}
% We also consider the scenario of accumulating a diverse range of videos which fall under an activity label umbrella. For this we look specifically at complex activities, and curated videos for 4 activities: vacuum cleaning, ironing, rope jumping, cycling

% %sources of videos ... details about how we selected the videos..

% In total, videos of 12 activities are studied. Their activity labels allow us to make direct comparison with three popular IMU-based datasets: Realworld, PAMAP2 and Opportuntiy. A random subject was chosen as the held out test set to report performance on, in realworld this is subject 15, in PAMAP2 subject 6, in Opportunity subject 4.

% Prior to passing any virtual data into the machine learning model for classification on real IMU data, we also apply a simply mapping technique to match the data distributions in both domains. more about the mapping technique...

% We employed three classes of machine learning methods for activity recognition in our experiments: random forests, DeepConvLSTM, and autoencoder-MLP. For the trianing of deep models, we followed standard hyperparameter tuning protocol of a grid search of learning rate from $10^{-6}$ to $10^{-3}$ and weight decay from $10^{-4}$ to $10^{-3}$ using a held out validation set. 

%---------------------
%--- Catherine
%--- Hyeok have reflected them.
% Classifiers were trained and tested using these protocols: Real-to-Real, Virtual-to-Real, Mixed-to-Real, Transfer learning. Under Real-to-Real, classifiers were trained using on real IMU data. Under Virtual-to-Real, classifiers were trained using virtual data only. Under Mixed-to-Real, classifiers were trained on a mixture of virtual and real data. Under Transfer learning, classifiers were pre-trained using the virtual data, then finetuned using real data. In all scenarios, we report using the performance on the held-out real test set. Reported scores are the mean of three runs initiated with different random seeds.

% % (combine into one big table)
% \textbf{Overview} {}

% % realworld data - holding activity constant 
% Performance on the realworld dataset is summarized in Table~\ref{fig:rw_overall} 
% Overall, models trained from virtual data alone achieves reasonable performance when tested on real data - around > 70\% of Real-to-Real
% This dip goes away when some labelled real data is used in the training process, not only that, using both virtual and real data helps.

% \vspace{0.5em}

% \textbf{How much real data is needed.} {}

% \vspace{0.5em}

% \textbf{Increasing train data size with virtual data.} {}
% Figure~\ref{fig:dl_mix2r} shows how the recognition results vary when the train data size is doubled by adding virtual data. Mixing data does not always help, e.g. in opportunity case. 

% \vspace{0.5em}

% \textbf{Better representation learning} {}
% In the deep learning case, transfer learning always outperform Real-to-Real and Mixed-to-Real. This shows potential in using virtual data for representation learning. 
% Also, transfer learning gives rise to a flexibility in label choice, since the final layer of the neural network can be replaced to incorporate any number of classes. The performance difference between a finetuned model pretrained from 8 and 11 classes is insignificant. 


==> sec_4/figures/dl_mix2r.tex <==
\begin{figure}[t!]
	\centering
	\begin{tabular}{c} 	
		\subfigure[RealWorld]{
			\includegraphics[width=0.45\linewidth]{sec_4/figures/dl_mix2r_rw.png}
			\label{fig:dl_mix2r_rw}
		}
		\subfigure[PAMAP-11]{
			\includegraphics[width=0.45\linewidth]{sec_4/figures/dl_mix2r_p11.png}
			\label{fig:dl_mix2r_p11}
		}
	\end{tabular} 
	\label{fig:dl_mix2r}
\end{figure}

==> sec_4/figures/rf_dl.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}[t]{@{\hspace{-0.25cm}}c c @{\hspace{-.10cm}}c}
    Realworld &
    \includegraphics[align=c,height=0.3\linewidth]{sec_4/figures/rw/rf_rw.png}\vspace{-0.1in} &
    \includegraphics[align=c,height=0.3\linewidth]{sec_4/figures/rw/dl_mix2r_rw.png}\vspace{-0.1in} \\
    PAMAP2-11 &
    \includegraphics[align=c,height=0.3\linewidth]{sec_4/figures/pmp/rf_pmp11.png}\vspace{-0.0in}&
    \includegraphics[align=c,height=0.3\linewidth]{sec_4/figures/pmp/dl_mix2r_p11.png}\vspace{-0.0in}\\
     & RF & ConvLSTM
\end{tabular}
\end{center}
\vspace{-0.15in}
\caption{The performance change according to virtual and real IMU training sample size. 
The R2R (real\_full) is trained with all the training sample size, whereas the others are trained with the sample size according to the x-axis.
For both datasets and models, M2R (vir\_sub + real\_sub) outperforms V2R (vir\_sub) models.
\textcolor{red}{Have to unify the color, legend}}
\label{fig:supervised} 
\vspace*{-1em}
\end{figure}

% \begin{figure}[t]
% \begin{center}
% \begin{tabular}[t]{@{\hspace{-1.85cm}}c @{\hspace{-0.75cm}}c}
%     RealWorld & Pamap-11\\
%     \begin{tabular}{c@{\hspace{-0.5cm}}c}
%         \includegraphics[valign=b,align=c,width=0.325\linewidth]{sec_4/figures/rw/rf_rw.png}\vspace{-0.0in} &  
%         \includegraphics[valign=b,align=c,width=0.325\linewidth]{sec_4/figures/rw/dl_mix2r_rw.png}\vspace{-0.0in} \\
%         RF & ConvLSTM
%     \end{tabular} &
%     \begin{tabular}{c@{\hspace{-0.5cm}}c}
%         \includegraphics[valign=b,align=c,width=0.325\linewidth]{sec_4/figures/pmp/rf_pmp11.png}\vspace{-0.0in} &  
%         \includegraphics[valign=b,align=c,width=0.325\linewidth]{sec_4/figures/pmp/dl_mix2r_p11.png}\vspace{-0.0in} \\
%         RF & ConvLSTM
%     \end{tabular}
% \end{tabular}
% \end{center}
% \vspace{-0.15in}
% \caption{The performance change according to virtual and real IMU training sample size. 
% The R2R (real\_full) is trained with all the training sample size, whereas the others are trained with the sample size according to the x-axis.
% For both datasets and models, M2R (vir\_sub + real\_sub) outperforms V2R (vir\_sub) models.
% \textcolor{red}{Have to unify the color, legend}}
% \label{fig:supervised} 
% \vspace*{-1em}
% \end{figure}

==> sec_4/figures/tl.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}[t]{@{\hspace{-0.25cm}}c c @{\hspace{-.10cm}}c}
    Realworld &
    \includegraphics[align=c,height=0.3\linewidth]{sec_4/figures/rw/tl_rw.png}\vspace{-0.1in} &
    \includegraphics[align=c,height=0.3\linewidth]{sec_4/figures/rw/unsupervised_tl_rw.png}\vspace{-0.1in} \\
    PAMAP2-11 &
    \includegraphics[align=c,height=0.3\linewidth]{sec_4/figures/pmp/tl_p11.png}\vspace{-0.0in}&
    \includegraphics[align=c,height=0.3\linewidth]{sec_4/figures/pmp/unsupervised_tl_p11.png}\vspace{-0.0in}\\
     & ST2R & UT2R
\end{tabular}
\end{center}
\vspace{-0.15in}
\caption{Transfer learning with supervised (ST2R) and unsupervised (UT2R) pre-training with virtual sensor dataset. The trained models are fine-tuned with the subset of real sensor dataset.
Overall, ST2R pretrained model adapts to target task more efficiently than random initialization. 
ST2R with approximately 10 minutes of real sensor can outperform R2R model trained with full real sensor dataset.
\textcolor{red}{What is x-axis?
Let's wait for Harish's result for UT2R}}
\label{fig:dl_tl} 
\vspace*{-1em}
\end{figure}

%--------------------------------------
% catherine
% \begin{figure}[t!]
% 	\centering
% 	\begin{tabular}{c} 	
% 		\subfigure[RealWorld]{
% 			\includegraphics[width=0.45\linewidth]{sec_4/figures/tl_rw.png}
% 			\label{fig:tl_rw}
% 		}
% 		\subfigure[PAMAP-11]{
% 			\includegraphics[width=0.45\linewidth]{sec_4/figures/tl_p11.png}
% 			\label{fig:tl_p11}
% 		}
% 	\end{tabular} 
% 	\label{fig:dl_tl}
% \end{figure}


==> sec_4/tables/all.tex <==
\begin{table}[t!]
	\centering
	\begin{tabular}{c||c||c|c|c|c|c}
		\hline
		Dataset & Model & R2R & V2R & M2R & ST2R & UT2R \\
		\hline\hline
		\multirow{2}{4em}{Realworld} &
		% realworld
		Random Forest & 0.6416 & 0.6321 & 0.7797 & -     &  78.89 \\
		\cline{2-7}
		&
		ConvLSTM  & 0.730  & 0.524  & 0.745  & 0.834 & - \\
		\hline\hline
		% pamap2-11
		\multirow{2}{5em}{PAMAP2-11} &
		Random Forest & 0.7635 & 0.6508 & 0.7077 & -     & 69.37\\
		\cline{2-7}
		&
		ConvLSTM  & 0.698  & 0.533  & 0.700  & 0.702 & - \\
		\hline\hline
		% opportunity
		\multirow{2}{5em}{Opportunity} &
		Random Forest & 0.8823 & 0.8493 & 0.9150 & -     & -\\
		\cline{2-7}
		&
		ConvLSTM  & 0.887  & 0.783  & 0.838  & 0.910 & - \\
		\hline\hline
	\end{tabular}
	\caption{Summary of activity recognition results (mean F1 score) on Realworld (8 classes), PAMAP2 (11 classes), and Opportunity dataset.
	R2R model is trained with full real sensor dataset.
	Overall, V2R model approximately shows 70\% performance of the corresponding R2R model.
	M2R model trained with additional 10 minutes of real sensor data allways outperforms V2R model, and performs similarly as R2R model. 
	Lastly, ST2R model outperforms all the other models.
	Rich sensor representation from supervised training with all available virtual sensor data provides effective intial model weight to queickly adapt with small real sensor samples (only 10 minutes). 
	\textcolor{red}{Need update after getting UT2R result.}
	} \label{tbl:summary}
	\vspace{-1.2em}
\end{table}

% %----------------------------------------
% % realworld
% \begin{table}[t!]
% 	\centering
% 	\begin{tabular}{c|c|c|c|c|c}
% 		\hline
% 		& R2R & V2R & M2R & ST2R & UT2R \\
% 		\hline
% 		Random Forest & 0.6416 & 0.6321 & 0.7797 & -     & -\\
% 		DeepConvLSTM  & 0.730  & 0.524  & 0.745  & 0.834 & - \\
% 		\hline
% 	\end{tabular}
% 	\caption{Summary of classifier results (mean F1 score) on Realworld test for 8-class activity recognition.} \label{tbl:rw_overall}
% 	\vspace{-1.2em}
% \end{table}

% % pamap2-11
% \begin{table}[t!]
% 	\centering
% 	\begin{tabular}{c|c|c|c|c|c}
% 		\hline
% 		& R2R & V2R & M2R & ST2R & UT2R \\
% 		\hline
% 		Random Forest & 0.7635 & 0.6508 & 0.7077 & -     & -\\
% 		DeepConvLSTM  & 0.698  & 0.533  & 0.700  & 0.702 & - \\
% 		\hline
% 	\end{tabular}
% 	\caption{Summary of classifier results (mean F1 score) on PAMAP2 test data for 11-class activity recognition.} \label{tbl:pmp_overall}
% 	\vspace{-1.2em}
% \end{table}

% % opportunity
% \begin{table}[t!]
% 	\centering
% 	\begin{tabular}{c|c|c|c|c|c}
% 		\hline
% 		& R2R & V2R & M2R & ST2R & UT2R \\
% 		\hline
% 		Random Forest & 0.8823 & 0.8493 & 0.9150 & - & -\\
% 		DeepConvLSTM  & 0.887 & 0.783 &0.838 & 0.910 & - \\
% 		\hline
% 	\end{tabular}
% 	\caption{Summary of classifier results (mean F1 score) on Opportunity test data for 4-class activity recognition.} \label{tbl:pmp_overall}
% 	\vspace{-1.2em}
% \end{table}



==> sec_4/tables/opp.tex <==
\begin{table}[t!]
	\centering
	\begin{tabular}{c|c|c|c|c|c}
		\hline
		& R2R & V2R & M2R & ST2R & UT2R \\
		\hline
		Random Forest & 0.8823 & 0.8493 & 0.9150 & - & -\\
		DeepConvLSTM  & 0.887 & 0.783 &0.838 & 0.910 & - \\
		\hline
	\end{tabular}
	\caption{Summary of classifier results (mean F1 score) on Opportunity test data for 4-class activity recognition.} \label{tbl:pmp_overall}
	\vspace{-1.2em}
\end{table}

==> sec_4/tables/pmp.tex <==
\begin{table}[t!]
	\centering
	\begin{tabular}{c|c|c|c|c|c}
		\hline
		& R2R & V2R & M2R & ST2R & UT2R \\
		\hline
		Random Forest & 0.7635 & 0.6508 & 0.7077 & -     & -\\
		DeepConvLSTM  & 0.698  & 0.533  & 0.700  & 0.702 & - \\
		\hline
	\end{tabular}
	\caption{Summary of classifier results (mean F1 score) on PAMAP2 test data for 11-class activity recognition.} \label{tbl:pmp_overall}
	\vspace{-1.2em}
\end{table}

==> sec_4/tables/rw.tex <==
\begin{table}[t!]
	\centering
	\begin{tabular}{c|c|c|c|c|c}
		\hline
		& R2R & V2R & M2R & ST2R & UT2R \\
		\hline
		Random Forest & 0.6416 & 0.6321 & 0.7797 & -     & -\\
		DeepConvLSTM  & 0.730  & 0.524  & 0.745  & 0.834 & - \\
		\hline
	\end{tabular}
	\caption{Summary of classifier results (mean F1 score) on Realworld test for 8-class activity recognition.} \label{tbl:rw_overall}
	\vspace{-1.2em}
\end{table}

==> sec_4/tables/tl.tex <==
\begin{table}[t!]
	\centering
	\begin{tabular}{ccccc}
		\hline
		& Real & Pre-trained from 11-classes & Pre-trained from 8-classes \\
		\hline
		DeepConvLSTM  &0.698 &0.702 & 0.701 \\
		\hline
	\end{tabular}
	\caption{Transfer learning results (mean F1 score) on PAMAP2 test data for 11-class activity recognition.} \label{fig:pmp_overall}
	\vspace{-1.2em}
\end{table}



\begin{table}[t!]
	\centering
	\begin{tabular}{cccc}
		\hline
		& R2R & V2R & MIX2R \\
		\hline
		Realworld  &0.8011 &0.5634 & 0.8415 \\
			O4  &0.8971 &0.7882 & 0.8970 \\
				P8  &0.7601 &0.5591 & 0.7346 \\
					P11  &0.7138 &0.5702 & 0.7372 \\
		\hline
	\end{tabular}
	\caption{} \label{tl4}
	\vspace{-1.2em}
\end{table}
